Semantic SLAM with Autonomous Object-Level Data Association

It is often desirable to capture and map semantic information of an environment during simultaneous localization and mapping (SLAM). Such semantic information can enable a robot to better distinguish places with similar low-level geometric and visual features and perform high-level tasks that use semantic information about objects to be manipulated and environments to be navigated. While semantic SLAM has gained increasing attention, there is little research on semanticlevel data association based on semantic objects, i.e., object-level data association. In this paper, we propose a novel object-level data association algorithm based on bag of words algorithm, formulated as a maximum weighted bipartite matching problem. With object-level data association solved, we develop a quadratic-programming-based semantic object initialization scheme using dual quadric and introduce additional constraints to improve the success rate of object initialization. The integrated semantic-level SLAM system can achieve high-accuracy object-level data association and real-time semantic mapping as demonstrated in the experiments. The online semantic map building and semantic-level localization capabilities facilitate semantic-level mapping and task planning in a priori unknown environment.

==> backup/front_end.tex <==
In this section we describe the steps of the front end of our system that are performed on as many camera frames as possible. 

\subsection{Object Detection}
Object detection is an essential part of the proposed semantic SLAM system as it is the source of all semantic information. We make use of an ROS implementation \cite{bjelonicYolo2018} of YOLOv3 \cite{redmon2018yolov3} for real-time object detector. For every processed RGB or grey image $I_t$, YOLOv3 outputs a set of semantic measurements $\mathcal{S}_t$. 
% Each semantic measurement $z_{k}$ provides the following formation: 
% \begin{itemize}
%     \item Object bounding box $b_k = [x_{k, min}, y_{k, min}, x_{k, max}, y_{k, max}]$.
%     \item Object class.
%     \item Corresponding confidence score.
% \end{itemize}
We discard semantic measurements with bounding boxes smaller than certain threshold as we deemed them to hold too little image content to be robustly tracked.

\subsection{ORB Extraction}
In the next step, we uses the bag of words algorithm to convert the image content inside bounding boxes into BoW vectors. This algorithm requires ORB features in the conversion, which will be extracted in this step. 
% While ORB features are not the chosen features for our system, they are still required to compute the bag of words vectors. 
For each ROI bounded by a bounding box, FAST corners are extracted at 8 scale levels with a scale factor of 1.2. Each scale level is divided in a grid, and corners are extracted in each cell to ensure a homogeneous distribution. The density of the corners remains the same; hence the number of corners extracted per ROI varies according to the area of the ROI. For ROI that is textureless or has low contrast and holds few corners, its corresponding semantic measurement and corners extracted in this ROI are discarded. The ORB descriptors are then computed for the remaining FAST corners.  

\subsection{Convert to BoW vectors}
Visual vocabulary is the discretization of the descriptor space and is used to convert the ORB features extracted in each bounding box to BoW vectors. It is structured as a tree with binary nodes that is created by $k$-medians clustering of training ORB descriptors. The leaves of the tree are the words of the visual vocabulary, weighted with the term frequency - inverse document frequency (tf-idf) according to their relevance in the training corpus. Words with fewer occurrences in the training images are deemed more discriminative and given a higher weight.
% Considering objects of different classes reside in bounding boxes, the same vocabulary may not generalize well. 
Instead of using a single vocabulary, we create vocabularies for every object class in our implementation. Our intention is to ensure that each vocabulary is uniquely suited to distinguish the image content in bounding boxes of a particular object classes.
Each vocabulary is built offline with $k = 5$ branches and $L = 5$ depth levels, yielding 3125 words. Those vocabularies are learned with the ORB descriptors extracted within the ground truth bounding boxes from the COCO dataset images \cite{lin2014microsoft}. 

When ORB features are extracted from a bounding box of certain object class, we employ matching visual vocabulary to convert them into BoW vector. For all the given ORB features, their descriptor vectors traverse the vocabulary tree from the root to the leaves, selecting at each level the nodes which minimizes the Hamming distance. The BoW vector is simply the weighted occurrence counts of the words, i.e., leaves.

\subsection{Object-Level Data Association}
Accurate data association is essential for robust SLAM. We use object-level data association  to match the incoming semantic measurements form YOLOv3 to registered objects in the map. Our method is a two-step frame-to-map matching, described as follows.

First, we determine the set of matching object candidates $\mathcal{T}^{ca}$ for a semantic measurement $z_k \in \mathcal{S}_t$. Recall in Section \ref{ssec:Keyframe}, each map object $\tau_j$ contains its class label. For a semantic measurement $z_k= \{b_k, c_k, s_k\}$, only objects with the same class label are considered. In other words, data association is performed for objects and semantic measurements with the same class label. This method can significantly reduce the search space. Admittedly, YOLOv3 could sometimes assign different class label to the same object in some corner cases, and performing data association in this fashion denies us the opportunity to correct this error. We further narrow down the search space by imposing geometric requirements on potential matching objects considering two cases:
\begin{itemize}
    \item The map object $\tau_j$ has quadric representation. In this case, the projection of the object quadric center should reside inside the bounding box of the semantic measurement $z_k$, as shown on the right frame of Fig. \ref{fig:DA geometry}.
    \item The map object $\tau_j$ does not have quadric representation. In this case, we make the following assumption: the 3D point corresponding to the center of the bounding box of the latest observation of $\tau_j$ should be projected inside the bounding box of $z_k$. Based on this assumption, the corresponding epipolar line should go through the bounding box of $z_k$. The epipolar line is represented by the real line on the right frame of Fig. \ref{fig:DA geometry}.
\end{itemize}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=.9\linewidth]{figures/DA_geometry.jpg}
  \caption{The geometric requirements imposed on matching object candidates}
  \label{fig:DA geometry}
\end{figure}

Once we have determined the set of matching object candidates $\mathcal{T}^{ca}$, we proceed to the second step of data association. For every map object $\tau_j \in \mathcal{T}^{ca}$, our system goes though semantic keyframes $K_i \in \mathcal{K}^{j}$. A $L_1$-score $s(\mathbf{v}_1, \mathbf{v}_2)$ is calculated between the BoW vector stored in the semantic keyframe $K_i$ and the BoW vector corresponding to the bounding box of the semantic measurement $z_k$. The maximum score among $\mathcal{K}^{j}$ is considered the data association score $c_{kj}$ between the semantic measurement $z_k$ and the map object $\tau_j$. Define $x_{kj}$ as the 0-1 decision variable:  
\begin{equation}
    x_{kj} = \begin{cases}
    1, & \text{if } z_{k} \text{ is assigned to } \tau_j\\
    0, & \text{otherwise.}
    \end{cases}
\end{equation}

The object-level data association is then formulated as a maximum weighted bipartite matching problem (assignment problem): 

\begin{align}
\label{eqn:AP}
    \argmax_{x_{kj}} & \sum_{\{k:z_k \in \mathcal{S}_t^{c}\}}\sum_{\{j:\tau_j \in \mathcal{T}^{ca}\}} c_{kj}x_{kj} \\
    \textrm{s.t.} &     \sum_{\{j:\tau_j \in \mathcal{T}^{ca}\}} x_{kj} \leq 1\text{,\quad} \sum_{\{k:z_k \in \mathcal{S}_t^{c}\}} x_{kj} \leq 1.
    \label{eq:constraint} 
\end{align}

The constraints \eqref{eq:constraint} mean that (a) each semantic measurement can only be assigned to at most one map object and some semantic measurements cannot be assigned to map objects because they are either from new objects that have not yet been observed or due to false detections;
%in other words, some semantic measurements are new objects that have not been observed before or false detections; 
and (b) each map object could only be associated with at most one semantic measurement.

The problem defined in (\ref{eqn:AP}) can be solved using a cost-scaling push-relabel algorithm \cite{goldberg1995efficient, goldberg1990finding, kennedy1995solving, burkard2012assignment, ahyja1993network}, readily implemented in \cite{ortools}. This algorithm has a time complexity of $\mathcal{O}(\sqrt{n}m\log{(nC)})$, where $n$ is the number of nodes in the bipartite graph, $m$ is the number of edges in the bipartite graph, and $C$ is the largest magnitude of an edge cost. 


% First, we use a greedy policy to match every semantic measurement $z_k \in \mathcal{S}_t$ to an map object $\tau_j$ without considering possible conflicts.
% % I feel this question is sufficiently addressed by the next paragraph and equation (5) and (6).
% % \todo[inline]{greedy with respect to what objective function? or some heuristics? clarify}
% Recall in Section  \ref{ssec:Keyframe}, each map object $\tau_j$ contains its class label. For a semantic measurement $z_k= \{b_k, c_k, s_k\}$, only objects with the same class label $\tau_j \in \mathcal{T}^{c_k}$ is considered. In other words, data association is performed for objects and semantic measurements with the same class label. This method can significantly reduce the search space. Admittedly, YOLOv3 could sometimes assign different class label to the same object in some corner cases, and performing data association in this fashion denies us the opportunity to correct this error.
% % since it is not supported, I willnot include this claim Nevertheless, we believe the gains in efficiency outweigh the potential loss in accuracy. 
% For every map object $\tau_j \in \mathcal{T}^{c_k}$, our system goes though semantic keyframes $K_i \in \mathcal{K}^{j}$. A $L_1$-score $s(\mathbf{v}_1, \mathbf{v}_2)$ is calculated between the BoW vector stored in the semantic keyframe $K_i$ and the BoW vector corresponding to the bounding box of the semantic measurement $z_k$.
% % \begin{equation}
% %     s(\mathbf{v}_1, \mathbf{v}_2) = 1 - \frac{1}{2}\bigg\lvert \frac{\mathbf{v}_1}{\lvert\mathbf{v}_1\rvert}-\frac{\mathbf{v}_2}{\lvert\mathbf{v}_2\rvert}\bigg\rvert
% % \end{equation}
% The maximum score among $\mathcal{K}^{j}$ is considered the data association score $c_{kj}$ between the semantic measurement $z_k$ and the map object $\tau_j$. The map object in $\mathcal{T}^{c_k}$ yielding the maximum data association score is considered the matching object to the semantic measurement. Define $x_{kj}$ as the 0-1 decision variable:  
% \begin{equation}
%     x_{kj} = \begin{cases}
%     1, & \text{if } z_{k} \text{ is assigned to } \tau_j\\
%     0, & \text{otherwise}
%     \end{cases}
% \end{equation}
% \noindent Mathematically, the greedy policy executed in the first step can be formulated as:
% \begin{equation}
%      \argmax_{x_{kj}}  \sum_{\{j:\tau_j \in \mathcal{T}^{c_k}\}} c_{kj}x_{kj} \text{,\quad}\textrm{s.t.}  \sum_{\{j:\tau_j \in \mathcal{T}^{c_k}\}} x_{kj} = 1
%      \label{eq:first step}
% \end{equation}

% The optimization problem defined in \eqref{eq:first step} is solved for every semantic measurement $z_k \in \mathcal{S}_t$. It should be noted that in the first step of frame-to-map matching, one map object can be matched to two or more semantic measurements. Hence, in the following second step of data association, such conflicts are detected and resolved. For the type of object class $c \in \mathtt{Conf}$ where conflicts do occur, the semantic measurements of object class $c$ is re-performed. In this step, instead of performing data association based on a greedy policy, we reformulate object-level data association as a maximum weighted bipartite matching (assignment problem): 

% \begin{align}
% \label{eqn:AP}
%     \argmax_{x_{kj}} & \sum_{\{k:z_k \in \mathcal{S}_t^{c}\}}\sum_{\{j:\tau_j \in \mathcal{T}^{c}\}} c_{kj}x_{kj} \\
%     \textrm{s.t.} &     \sum_{\{j:\tau_j \in \mathcal{T}^{c}\}} x_{kj} \leq 1\text{,\quad} \sum_{\{k:z_k \in \mathcal{S}_t^{c}\}} x_{kj} \leq 1
%     \label{eq:constraint} 
% \end{align}

% The constraints \eqref{eq:constraint} mean that (a) each semantic measurement can only be assigned to at most one map object and some semantic measurements cannot be assigned to map objects because they are either from new objects that have not yet been observed or due to false detections;
% %in other words, some semantic measurements are new objects that have not been observed before or false detections; 
% and (b) each map object could only be associated with at most one semantic measurement, 
% %in other words, some map objects would not be associated with any semantic measurements because they are not observed in the current frame. 
% Conflicts occurred in the first step of data association is a violation of the second requirement. By satisfying those two constraints during the second step of data association, the conflicts are resolved. 

% The problem defined in (\ref{eqn:AP}) can be solved using a cost-scaling push-relabel algorithm \cite{goldberg1995efficient, goldberg1990finding, kennedy1995solving, burkard2012assignment, ahyja1993network}, readily implemented in \cite{ortools}. This algorithm has a time complexity of $\mathcal{O}(\sqrt{n}m\log{(nC)})$, where $n$ is the number of nodes in the bipartite graph, $m$ is the number of edges in the bipartite graph, and $C$ is the largest magnitude of an edge cost. The time complexity of this algorithm is 
% significantly higher than that of the greedy policy implemented in the first step, $\mathcal{O}(m)$. Considering that the greedy policy has superior efficiency, and conflicts in data association rarely happens during the first step even without explicitly specifying the constraints, we adopt this two-step object-level data association scheme. 

\subsection{New Semantic Keyframe Decision}
\label{ssec:NSKDecision}
The last step in our front end is to decide whether the current frame should be spawned as a new semantic keyframe. Currently, one out of every four frame is chosen as the semantic Keyframe. This is a rather naive implementation and more sophisticated criteria will be developed in future work to ensure good tracking. If a semantic keyframe is inserted when the semantic mapping is busy, a signal is sent to stop bundle adjustment, so that the semantic mapping thread can process the new semantic keyframe as soon as possible.
% Since a culling mechanism is implemented in the mapping thread to remove redundant semantic keyframes, semantic keyframes are inserted as fast as possible to ensure robust tracking. The following three conditions must be met before a new semantic keyframe can be inserted: 
% \begin{enumerate}
%     \item Mapping is idle, or more than 20 frames have passed from last semantic keyframe insertion.
%     \item New map object is observed in the current frame if a semantic measurement in the current frame is not associated with a map object after performing data association or its corresponding data association score is smaller than a threshold.  
%     \item The data association score of certain objects in the current frame falls below ....
% \end{enumerate}

% Conditions 2) and 3) ensure good tracking. 




==> backup/system_overview.tex <==
\subsection{Overview of Semantic SLAM System}
\begin{figure}[htbp]
  %\centering
  \includegraphics[width=1\linewidth]{figures/System Overview.jpg}
  \caption{System overview, showing all the steps performed in semantic object detection and tracking thread and semantic mapping thread. The main components of the map are also shown.}
  \label{fig:system overview}
\end{figure}
%  Figure~\ref{fig:system overview} presents an overview of our system composed of two threads: semantic object detection and tracking (Sec.~\ref{sec:Front End}) and semantic mapping (Sec.~\ref{sec:Mapping}). The map contains a set of map objects and semantic keyframes, as well as the correspondence between them.   A semantic keyframe stores the map objects it has observed in the frame image. At the same time, each map object records the sequence of semantic keyframes in which this object has been observed. Similar to \cite{nicholson2018quadricslam}, our semantic SLAM employs semantic objects as landmarks and represents them as dual quadrics.  The representations of objects, as well as the attributes of map objects and semantic keyframes can be found in the Appendix.  Next, we provide more details about the algorithms used in these two threads.

We now present an overview of our system that integrate object detection, semantic-level data association, and bundle adjustment into SLAM for meaningful semantic mapping and localization.
The system overview is shown in Fig. \ref{fig:system overview}. The incoming 
video frames or images $\mathcal{I}$ are fed into the front-end of our algorithm. In the front-end, objects are detected in an incoming frame and then matched to objects already registered in the map, i.e., object-level data association is performed. The decision to insert new semantic keyframe is also made in this part, and a new semantic keyframe is subsequently generated. Triggered by the new semantic keyframe, the main task of the semantic mapping thread is to perform joint SLAM optimization of semantic keyframe poses and map objects, and to maintain the set of objects in the map. 

The front-end processes all the incoming video frames. The incoming frames are first processed by two modules running in parallel. One module is object detection. YOLOv3 \cite{redmon2018yolov3} is used in the object detection module to detect objects presented in the current frame. The other module is SLAM tracking, which provides the pose estimation of the current frame. We use the tracking thread of orb\_slam2 \cite{mur2017orb} for this purpose. Oriented FAST and rotated BRIEF (ORB) features are then extracted in the Region of Interest (ROI) of the current frame and converted to Bag of Words (BoW) vectors. Data association is subsequently performed based on the  geometric location of the map objects and matching score between the BoW vectors in the current frame and that of the objects in the map. 

%The current frame will be deemed as a semantic keyframe if it satisfies certain criterion detailed in \ref{ssec:NSKDecision}.

The semantic mapping thread is triggered by a new semantic keyframe. In this thread, if consistent observations of a new object are made, the new object is initialized in the map. The map thread also includes a bundle adjustment module based on g2o \cite{kummerle2011g} which jointly optimizes objects and semantic keyframe poses.  

\subsection{Feature Choice}
In vision-based geometric SLAM, features such as ORB \cite{orb}, SIFT\cite{Sift} and SURF \cite{surf} are used in mapping, tracking and place recognition. Those features describe the interested points on the image and are sufficient for building a map of point clouds. In our semantic SLAM approach, we need to describe objects instead of points, and hence need to use different kind of features (i.e., image descriptors) such as DBoW2 \cite{galvez2012bags}, VLAD \cite{arandjelovic2013all} and Fisher \cite{van2014fisher}, which describe a ROI where an object resides. 
%Leveraging between speed and performance, 
To achieve a balance between speed and performance, we currently chose DBoW2 with ORB in our system. This is because that the mean execution time of this feature per extraction is smaller than 20 ms. Under the current framework, it is possible to switch to other features should faster and more representative features emerge in the future. 

\subsection{Object Representation}
\label{ssec:objrep}
We represent semantic objects in a map as dual quadrics. A quadric, 
% in its primal form, is represented by the locus of all points $M$ on the surface 
% %of the quadric
% \xiao{defined by a quadratic equation}:
% \begin{equation}
%     M^T\mathbf{Q}M=0
% \end{equation}
% where $\mathbf{Q}$ is a $4 \times 4$ symmetric matrix only defined up to scale. A quadric thus depends on nine independent parameters.
in its dual form, is represented by the locus of all planes  that are tangent to the quadric. A tangent plane $\Pi$ satisfies:
\begin{equation}
    \Pi^T\mathbf{Q}^*\Pi=0
    \label{eq:quadric def}
\end{equation}
where ${\bf Q}^*$ is a $4 \times 4$ symmetric matrix defining a quadric and only defined up to scale, and  
$\Pi$ is a $4\times 1$ vector corresponding to the coefficients of general form of the plane equation. Note that coefficients of plane equations are the parametrization of all planes mentioned in this paper.

While quadrics can be used to represent both closed surfaces, for instance, ellipsoids, and open surfaces, such as paraboloid, hyperboloid, cone and cylinder, in this paper, we only consider ellipsoids to represent objects. Following \cite{rubino20173d}, the dual quadric of an ellipsoid is parameterized as:
\begin{equation}
    \mathbf{Q}^{*} =\mathbf{Z}\breve{\mathbf{Q}}^*\mathbf{Z}^T
\label{eq:ellipsoid}
\end{equation}
where $\breve{\mathbf{Q}}^*$ is an ellipsoid centred at the origin and with the principal axes aligned to the 3D coordinates, and $\mathbf{Z}$ is a homogeneous transformation that accounts for an arbitrary rotation and translation:
\begin{equation}
\mathbf{Z} = 
\begin{bmatrix}
    \mathbf{R} & t \\
    0_3^T     & 1
\end{bmatrix}
\text{,\quad}
\breve{\mathbf{Q}}^*=
\text{diag}(a^2, b^2, c^2, -1)
\end{equation}
where $t = [t_1, t_2, t_3]^T$ is the translation vector, $\mathbf{R}$ is the $3\times 3$ rotation matrix and $a, b, c$ are the three semi-axes of the ellipsoid.

\subsection{Associating Objects and Semantic Keyframes}
\label{ssec:Keyframe}
%Inspired by the implementation method between keyframes and map points in ORB-SLAM2 \cite{mur2017orb}, We build the relationship between 
In this section, we establish correspondences between semantic keyframes and objects. A semantic keyframe stores the map objects it has observed in the frame image, while each map object records the semantic keyframes that have observed the object sequentially. Those correspondences can then be quickly retrieved for object-level data association, object initialization and bundle adjustment. All detected objects and semantic keyframes are stored in the map.

In each map object $\tau_j$, the following attributes are stored:
\begin{itemize}
  \item Shape of the quadric represented  by three semi-axes: $a$, $b$, $c$.
  \item Rotation matrix of the quadric $\mathbf{R}$.
  \item Translation of the quadric $o_{\tau_j} = t$.
  \item The class label of the object.
  %and the corresponding confidence score.
  \item The set of semantic keyframes $\mathcal{K}^{j}$ that can observe this object.
  \item The number of observations.
\end{itemize}

Each Semantic keyframe $K_i$ stores the following information:
\begin{itemize}
  \item The camera pose $\mathbf{T}^i_w$ representing the world frame with respect to the camera frame, in terms of a homogeneous transformation matrix.
  \item The camera intrinsics, including focal length and principal point.
  \item Objects that have been observed in this semantic keyframe.
%   \item The bounding \xiao{box that contains the observed map objects in the keyframe}: Object bounding boxes $\{b_k\},k=1,2,\dots$. 
% %   \xiao{***JX: Just one bounding box or a bounding box for each object? If latter, just one $b$ is not sufficient. ***}
%   \item The class labels of the observed map objects.
  \item The set of semantic measurements taken at the this frame, associated or not to a map object.
  \item BoW vectors for the ROI defined by bounding boxes, used to describe observed map objects.
\end{itemize}

% \todo[inline]{Is BoW clear to all audience? If not, you could include a paragraph to describe it.}
% I feel like my description in Section V. C addresses this.

% % Similar to  ORB-SLAM2 \cite{mur2017orb}, Map objects and semantic keyframes are created with a generous policy. In a later stage, a very exigent culling mechanism is implemented to detect redundant semantic keyframes and wrongly matched or not trackable map objects. Culling procedures of map objects and semantic keyframes are explained in Sections \ref{ssec:Objects Culling} and  \ref{ssec:keyframe culling} respectively.
    


==> bibtex/section/objTracking.tex <==
\subsection{Object Tracking}
Tracking the trajectory of an object or Object tracking can be defined as associating information of a particular set of objects throughout a sequence of Images. In recent years multiple methods have been developed to robustly track multiple objects using visual using different sensors such as lidar based \cite{objlidar}, stereo camera \cite{objstereo} and monocular camera \cite{objref3}. In this work we focus mainly on vision based tracking/ monocular image based object tracking \cite{objref1}, \cite{objref2}, \cite{objref3}. The problem of object tracking can be divided into three important steps which are object detection, object representation and object data association \cite{survey_objdet}. In our work, we use YOLOv3 for the object detection part. For the object representation part, instead of shape \cite{objrep1} or appearance\cite{objrep2} based representations we use BoW algorithm to create word vectors of the object (explained in detail in \ref{sec:System Overview}). For the object association we use a customized tracking algorithm which uses the BoW vector representations to track multiple objects in real-time.

==> bibtex/section/problem_formulation.tex <==
\newtheorem*{N5}{Images}
\begin{N5}
Our inputs are a set of images $\mathcal{I} = \{I_t\}_{t=0}^T$, where $I_t$ is the image taken at time instance $t$.
\end{N5}

\newtheorem*{N4}{Objects}
\begin{N4}
We use $\mathcal{T} = \{\tau_j\}_{j=1}^{N}$ to represent the $N$ objects registered in the map.
% Let $\mathcal{C}$ be the set of object classes, $\mathcal{T}^c \subset \mathcal{T}$ is the set of objects with class $c \in \mathcal{C}$. 
The specific definition of an object $\tau_j$ can be found in \ref{ssec:Keyframe}.
\end{N4}

\newtheorem*{N6}{Semantic Keyframes}
\begin{N6}
We use $\mathcal{K} = \{K_i\}_{i=1}^{P}$ to represent the $P$ semantic keyframes registered in the map. $\mathcal{K}^{j}$ stands for the set of semantic keyframes that share the observation of the same object $\tau_j$. The specific definition of a semantic keyframe $K_i$ can be found in \ref{ssec:Keyframe}.
\end{N6}

\newtheorem*{N1}{Odometry measurements}
\begin{N1}
$u_t \in \mathbf{SE}(3)$ is the odometry taken at time instance $t$, describing the relative pose change in time interval $[t-1, t]$. Let $\mathcal{U} = \{u_t\}_{t=1}^T$ be the collection of all odometry measurements.
\end{N1}

\newtheorem*{N3}{Bounding box}
\begin{N3}
A bounding box $b_k$ is defined by two opposite corners: $b_k = [x_{k, min}, y_{k, min}, x_{k, max}, y_{k, max}]$. 
\end{N3}

\newtheorem*{N2}{Semantic measurements}
\begin{N2}
$z_k = \{b_k, c_k, s_k\}$ is $k$-th semantic measurement. It is a collection of three attributes, i.e., bounding box $b_k$, object class $c_k$, and detection score $s_k$. $\mathcal{S} = \{z_k\}_{k=0}^M$ is the collection of all semantic measurements.
% $\mathcal{S}_i \subset \mathcal{S}$ is the set of semantic measurements taken on semantic keyframe $K_i$.
$z_{K_i}^{\tau_j}$ is the semantic measurements taken on semantic keyframe $K_i$ of object $\tau_j$. Let $\mathcal{S}_t$ be the set of semantic measurements taken on image $I_t$ and $\mathcal{S}_t^c \subset \mathcal{S}_t$ be the set of semantic measuremnts taken on image $I_t$ with class $c$.
\end{N2}

\newtheorem*{N7}{Sensor state trajectory}
\begin{N7}
A sensor state trajectory is a sequence of all camera poses associated with semantic keyframes: $\mathcal{X} = \{x_i = T^i_w\}_{i=1}^{P}$, where $T^i_w \in \mathbf{SE}(3)$ describes the position and orientation of the camera.
\end{N7}
% \todo[inline]{ADD TRANSITION PARAGRAPH:
% In this work, we will develop a semantic SLAM algorithm with... }
In this work, we will develop a semantic SLAM algorithm with odometry measurements $\mathcal{U}$ and semantic measurements $\mathcal{S}$ generated from monocular images $\mathcal{I}$. The problem can be put as:
\newtheorem*{Problem}{Problem}
\begin{Problem}
Given odometry measurements $\mathcal{U}$ and semantic measurements $\mathcal{S}$, estimate the sensor state trajectory $\mathcal{X}$ and the pose, size, and classes of objects $\mathcal{T}$ in the environment.
\end{Problem}

Formally, this problem can be formulated as a Maximum a posteriori (MAP) estimation:
\begin{equation}
\begin{split}
    \mathcal{X}^*, \mathcal{T}^* & = \argmax_{\mathcal{X}, \mathcal{T}} p(\mathcal{X}, \mathcal{T}\;|\;\mathcal{U}, \mathcal{S}) \\ & =\argmax_{\mathcal{X}, \mathcal{T}} p(\mathcal{U}, \mathcal{S}\;|\;\mathcal{X}, \mathcal{T}) p(\mathcal{X})p(\mathcal{T}).
\end{split}
\label{eq:problem formulation}
\end{equation}
In \eqref{eq:problem formulation}, $p(\mathcal{U}, \mathcal{S}\;|\;\mathcal{X}, \mathcal{T})$ is the likelihood of the measurements $\mathcal{U}$ and $\mathcal{S}$ given the assignment $\mathcal{X}$ and $\mathcal{T}$. $p(\mathcal{X})$ and $p(\mathcal{T})$ are prior probabilities over $\mathcal{X}$ and $\mathcal{T}$.

With perfect data association, \eqref{eq:problem formulation} can be factored as:
\begin{equation}
\begin{split}
     \mathcal{X}^*, \mathcal{T}^*  = & \argmax_{\mathcal{X}, \mathcal{T}} 
      \underbrace{\prod_{i=1}^{P-1} p(u_{i+1}\;|\;x_{i+1}, x_i)}_{\text{Odometry}} \cdot \\
     & \underbrace{\prod_{j=1}^{N}\prod_{\{i:K_i \in \mathcal{K}^{j}\}} p(z_{K_i}^{\tau_j}\;|\;x_i, \tau_j)}_{\text{Semantic}} \cdot\underbrace{\prod_{j=1}^{N}p(\tau_j)}_{\text{Object Prior}}\cdot \underbrace{\prod_{i=1}^{P} p(x_i)}_{\text{Pose Prior}}.
     \label{eq:factor graph}
\end{split}
\end{equation}

In previous work of semantic SLAM, the data-association problem is assumed to be pre-solved \cite{nicholson2018quadricslam, ok2019robust} or rely on pre-built object database \cite{salas2013slam++, galvez2016real}, justifying the conversion from \eqref{eq:problem formulation} to \eqref{eq:factor graph}. However, such information is generally not readily available in real world applications. Hence, in our work, we solve the data association problem on the fly and still make \eqref{eq:factor graph} a valid approximation of \eqref{eq:problem formulation}.
